10 Years of Fair Representations: Challenges and Opportunities

Fair Representation Learning (FRL) is a broad set of techniques, mostly based on neural networks, that seeks to learn new representations of data in which sensitive or undesired information has been removed. Methodologically, FRL was pioneered by Richard Zemel et al. about ten years ago. The basic concepts, objectives and evaluation strategies for FRL methodologies remain unchanged to this day. In this paper, we look back at the first ten years of FRL by i) revisiting its theoretical standing in light of recent work in deep learning theory that shows the hardness of removing information in neural network representations and ii) presenting the results of a massive experimentation (225.000 model fits and 110.000 AutoML fits) we conducted with the objective of improving on the common evaluation scenario for FRL. More specifically, we use automated machine learning (AutoML) to adversarially "mine" sensitive information from supposedly fair representations. Our theoretical and experimental analysis suggests that deterministic, unquantized FRL methodologies have serious issues in removing sensitive information, which is especially troubling as they might seem "fair" at first glance.

==> experiments.tex <==
\section{Experiments}

In this section, we report on an in-depth experimentation that we conducted with the aim of evaluating the significance of the impossibility theorem stated in the previous section.
We are especially interested in testing whether it is still possible to predict the sensitive attribute $S$ with a high degree of accuracy from the fair representations learned by deterministic FRL methodologies, as our theoretical result suggests that it should be so.
To this end, we evaluated a total of 8 FRL methodologies: BinaryMI and DetBinaryMI, \cite{cerrato2023invariant}, DebiasClassifier \cite{ganin2016jmlr,xie2017controllable,madras}, NVP \cite{fairNVP}, VFAE \cite{Louizos2016TheVF}, ICVAE \cite{moyer2018invariant}, LFR \cite{zemel2013learning} and Deep Domain Confusion \cite{tzeng2014deep}.
While some of these are fully determinisic, others incorporate stochasticity by sampling from a parametric distribution which parameters are learned in the network.
Our expectation is that stochastic models will show greater invariance in their learned representations, as Theorem \ref{th:theorem1} does not apply and sensitive information may in principle be removed.
We tested these models on six different commonly employed fairness-sensitive datasets, focusing on the task of fair classification and independence as a fairness definition (i.e. $\hat{Y} \bot S$). 
We give in-depth descriptions of models and datasets in the Appendix, Sections~\ref{sec:app-models} and \ref{sec:app-datasets}, respectively.

We release \texttt{EvalFRL}\footnote{\url{https://anonymous.4open.science/r/EvalFRL/}}, the experimental framework we employed to perform our experimentation alongside all experimental metadata, including best hyperparameters for all models and performance at the outer fold level\footnote{\url{https://drive.google.com/drive/folders/1koZd8cgBJMVGuH3uRqvpTFEUJo0Sd23q?usp=sharing}} \footnote{We discuss the used compute infrastructure to run the experiments in the Appendix \ref{sec:compute}.}. Our framework was developed to perform in-depth evaluation of FRL methodologies across the two main frames discussed in Section \ref{sec:challenge} -- fair allocation and invariant representations. Thus, we evaluate both the fairness of the allocations learned by FRL methods and approximate the mutual information between the representations $Z$ and the sensitive attribute $S$ with the performance of external estimators.
%
%\textcolor{red}{What datasets, what models, what metric etc.}
%
\subsection{\texttt{EvalFRL}: An Evaluation Library for Fair Representation Learning}
%The empirical analysis revolves around the key idea of leveraging supervised learning techniques to predict the sensitive information $S$ of an individual, using fair representations generated by the FRL algorithms.
%With this adversarial approach the performance of this estimator of $S$ can be used as an approximation of the mutual information $I(Z;S)$. \textcolor{purple}{Maybe the word "approximation" is too strong, since e.g. the accuracy is between 0 and 1, while the mutual information is given in bits?}
As mentioned above, if an estimator can predict $S$ better than random guessing, this indicates that information on $S$ is still contained in the fair representation.
To investigate whether this may happen in commonly employed FRL techniques, we developed the \texttt{EvalFRL} framework, wherein every tested dataset-model combination follows a standardized testing pipeline.
This process is fully reproducible, thereby ensuring comparability between the models.
%
%The quality of the approximation strongly depends on the used estimator. 
%It can happen that due to e.g. the selection of an unsuitable model or a narrow training process, the estimator underperforms and the FRL model appears fairer.
In previous work tackling FRL, the experimental setup has focused on training a few classifiers on $(Z^i, S)$ \cite{cerrato2020constraining,zemel2013learning,Louizos2016TheVF,xie2017controllable}. 
However, the number of classifiers may vary and the optimal hyperparameters are not always reported, leading to results which are hard to compare across different papers.
We employ automated machine learning (AutoML) to handle this problem.
AutoML automatically searches for the optimal machine learning solution for a given problem.
This includes, among others, feature preprocessing, model selection and hyperparameter tuning. 

\begin{algorithm}
    \caption{Overview of \texttt{EvalFRL} logic when ran for one dataset-model combination.}
    \label{alg:framework}
    \begin{algorithmic}
        \State $\textcolor{goodblue}{r} \gets 15$, $\textcolor{goodblue}{k} \gets 3$, $\textcolor{goodblue}{seed} \gets 123$, $\textcolor{goodblue}{results} \gets []$, $\textcolor{goodblue}{repr_{\text{train}}} \gets []$, $\textcolor{goodblue}{repr_{\text{test}}} \gets []$
        \For{$i$ \textcolor{goodblue}{in} $1$ \textcolor{goodblue}{to} $r$}
            \State $X_{\text{train}}, X_{\text{test}}, y_{\text{train}}, y_{\text{test}}, s_{\text{train}}, s_{\text{test}} \gets \text{\textsc{train\_test\_split}}(X, y, s, \frac{2}{3}, \text{random\_state} = seed)$
            \State $cv \gets \text{\textsc{RandomizedSearchCV}}(model, param\_distributions, cv=k, n\_iter=100)$
            \State $\text{\textsc{bestmodel}} \gets cv.\text{\textsc{fit}}(X_{\text{train}}, y_{\text{train}}, s_{\text{train}}, \gamma=0)$
            \For{$\gamma_0$ \textcolor{goodblue}{in} $\{0, 0.1, \dots 1\}$}
                \State $\text{\textsc{bestmodel.fit}}(X_{\text{train}}, y_{\text{train}}, s_{\text{train}}, \gamma=\gamma_0)$ \Comment{\textcolor{goodgreen}{bestmodel is fit from scratch}}
                \State $results.\text{\textsc{append}}(\text{\textsc{evaluation}}(\text{\textsc{bestmodel}}, X_{\text{test}}, y_{\text{test}}, s_{\text{test}}))$
                \State $repr_{\text{train}}.\text{\textsc{append}}(\text{\textsc{get\_representations}}(\text{\textsc{bestmodel}}, X_{\text{train}}))$
                \State $repr_{\text{test}}.\text{\textsc{append}}(\text{\textsc{get\_representations}}(\text{\textsc{bestmodel}}, X_{\text{test}}))$
            \EndFor
            \For{$repr_{train_i}$, $repr_{test_i}$ \textcolor{goodblue}{in} ($repr_{\text{train}}, repr_{\text{test}}$)}
                \State $AutoML \gets \text{\textsc{automl}}()$ \Comment{\textcolor{goodgreen}{AutoML is trained from scratch at each CV iteration}}
                \State $AutoML.\text{\textsc{fit}}(repr_{train_i}, s_{\text{train}})$
                \State $results.\text{\textsc{append}}(\text{\textsc{evaluation}}(AutoML, repr_{test_i}, s_{\text{test}}))$
            \EndFor
        \EndFor
    \end{algorithmic}
\end{algorithm}

We show in Algorithm \ref{alg:framework} the main use case of \texttt{EvalFRL}.
A detailed description of the steps and a graphical representation of the framework's logic is shown in the Appendix \ref{app:exp}.
The whole pipeline is built using the Kedro framework \cite{Alam_Kedro_2024} and can be easily extended to include other models, datasets and metrics beyond the ones we consider in this work.
The data preprocessing step starts with the segmentation of the data into features $X$, the label $y$ and the sensitive attribute $S$.
Additionally, $y$ gets transformed to either a positive ($y=1$) or a negative ($y=0$) outcome and $S$ to either the privileged ($S=1$) or underprivileged ($S=0$) group.
Categorical features undergo encoding, while continuous features are normalized with mean 0 and variance 1.
%
In the subsequent step, hyperparameter-tuning is performed utilizing $r$-times $k$-fold cross-validation \cite{bouckaertfrank2004}.
In our experiments we set $r=15$ and $k=3$ by following the recommendations in Naudeau and Bengio \cite{nadeau2003inference}.
The best hyperparameters found in every outer-loop, along with a range of $\gamma$ values regulating the fairness/accuracy tradeoff (Equation \ref{eq:tradeoff}), are then utilized to evaluate the model.
The evaluation step contains the model's predictive performance on the label $y$ (Acc, AUC), as well as multiple fair allocation metrics.
%
Finally, we seek to evaluate $Z$ and $S$, for each fair representation generated in the previous step.
We utilize an AutoML library called MLJAR \cite{mljar} for this process.
AutoML searches the best model and trains it using the representations on the train-data and the corresponding sensitive information $S$.
Its performance gets tested using the representations on the held out test data and $S$.

The output of the framework allows for an exploration of the trade-off between predicting the label $y$ and the fairness of the model according to known fairness-metrics.
Additionally, it provides researchers with a common, high-effort evaluation framework for FRL methodologies in the invariant representation framing. 
If it is possible to have a higher performance than guessing $S$ randomly, this leads to the conclusion that there is still information on $S$ contained in the representation.
These investigations are done over a range of $\gamma$ tradeoff values, which makes it possible to understand the impact of the $\gamma$ parameter on both representation invariance and fairness of allocations.
%
\subsection{Fairness Metrics}
% \paragraph*{Statistical Parity Difference}
% Statistical Parity Difference (SPD) measures the difference in the probability of favorable outcomes between protected and unprotected groups.
% It is defined as:

% \begin{equation}
% \text{SPD} = P(\hat{Y} = 1 \mid S = 0) - P(\hat{Y} = 1 \mid S = 1)
% \end{equation}
% where $\hat{Y}$ is the predicted outcome, and $S$ is the sensitive attribute (e.g., gender, race).
% A value of 0 indicates perfect fairness, while values closer to -1 or 1 indicate higher disparity.
\paragraph*{Area under Discrimination Curve (AUDC)}
We quantify disparate impact through discrimination, following the approach introduced by Zemel et al. \cite{zemel2013learning}.
The discrimination metric, denoted as $\text{yDiscrim}$, is defined as:

\begin{equation}
    \text{yDiscrim} = \left | \frac{\sum^n_{n:s_n=1} \hat{y}_n}{\sum^n_{n:s_n=1} 1} - \frac{\sum^n_{n:s_n=0} \hat{y}_n}{\sum^n_{n:s_n=0} 1} \right |,
\end{equation}
where $n:s_n=1$ indicates that the $n$-th example has a value of $s$ equal to 1.
%
To generalize this metric akin to how accuracy generalizes to obtain a classifier's area under the curve (AUC), we evaluate the above measure for different classification thresholds and then compute the area under this curve.
In our experiments, we utilized $100$ equispaced thresholds.
We call this measure AUDC, following conventions established in the literature \cite{interFair}.
Unlike AUC, lower values are indicative of better performance.
%
\paragraph*{rND}
To measure fairness in learning to rank applications, we use the rND metric~\cite{ke2017measuring}.
This metric evaluates differences in exposure across multiple groups and is defined as:
\begin{equation}
\text{rND} = \frac{1}{Z} \sum_{i \in \{10, 20, ...\}}^N \frac{1}{\log_{2}(i)} \left| \frac{ \mid S^{+}_{1...i} \mid}{i} - \frac{\mid S^+ \mid}{N} \right |.
\end{equation}
rND measures the difference between the ratio of the protected group in the top-$i$ documents and in the overall population.
The maximum value, $Z$, serves as a normalization factor and is computed with a dummy list where all members of the underprivileged group are placed at the end, representing ``maximal discrimination.''
The metric also penalizes over-representation of protected individuals at the top compared to their overall population ratio.
\subsection{Results in Fair Allocation}\label{sec:results-fair-alloc}
%
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/auc_discrimination_ACC_model_gamma_results_relu_False.pdf}
    \caption{Accuracy vs. 1 - AUC-Discrimination tradeoff for all six dataset and eight model combinations. Each model is displayed for different $\gamma$ values indicated via a colored point inside the model marker.}
    \label{fig:model-acc-auc-dis}
\end{figure}
The model accuracy vs. fairness tradeoff results are shown in Figure \ref{fig:model-acc-auc-dis} (ACC vs. 1-AUDC) and \ref{fig:model-auc-auc-dis} (AUC vs. 1-AUDC), as well as in Figure \ref{fig:model-acc-dis} (ACC vs. 1-Discrimination), \ref{fig:model-auc-dis} (AUC vs. 1-Discrimination), \ref{fig:model-acc-parity} (ACC vs. Statistical Parity Difference), \ref{fig:model-auc-parity} (AUC vs. Statistical Parity Difference), \ref{fig:model-acc-delta} (ACC vs. Delta), \ref{fig:model-auc-delta} (AUC vs. Delta), \ref{fig:model-acc-rnd} (ACC vs. 1-rND), \ref{fig:model-auc-rnd} (AUC vs. 1-rND) of the appendix. 
Each figure shows all combinations of the six datasets and eight models.
The colored points in the symbols of the models show the used $\gamma$ value, while the colored areas show the variance employing 100 Gaussian bootstrapping fits using the mean and variance of the model performance optained from the 15 hold-out splits.
%
For most datasets and metric combinations (e.g. Adult, Banks and German) one can observe that the performance of the the majority of the models is equal.
Most models show a well defined tradeoff behaviour when changing the $\gamma$ value.

In Figure \ref{fig:model-acc-auc-dis} we observe that the performance for the DebiasClassifier on the Compas dataset outperforms all other models.
However, it takes mostly fair allocation decisions at higher values of gamma.
We conclude that the performance of FRL methodologies in the task of fair allocation is approximately equal. Varying the tradeoff parameter $\gamma$, as expected, leads to fairer decisions.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/auc_discrimination_AUC_model_gamma_results_relu_False.pdf}
    \caption{AUC vs. 1 - AUC-Discrimination tradeoff for all six dataset and eight model combinations. Each model is displayed for different $\gamma$ values indicated via a colored point inside the model marker.}
    \label{fig:model-auc-auc-dis}
\end{figure}

\subsection{Results in Invariant Representations}\label{sec:invariant}
%
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/automl_AUC_pure_gamma_results_relu_False.pdf}
    \caption{AutoML AUC vs. gamma results for all six dataset and eight model combinations.}
    \label{fig:automl-acc}
\end{figure}
We now take the same models reported in the previous subsection and investigate whether AutoML is able to recover information about the sensitive attributes from their representations.
Here, we expect that the accuracy of AutoML will approach the proportion of the majority group in the dataset (Figure \ref{fig:automl-acc}), and that the AUC will approach 0.5 (Figure~\ref{fig:automl-auc}), as the tradeoff parameter $\gamma$ increases. 
The results are particularly striking: while this is indeed what happens for stochastic or quantized models (BinaryMI, DetBinaryMI, VFAE, ICVAE) at higher $\gamma$ values, deterministic models have serious issues removing information (DebiasClassifier, NVP, DeepDomainConfusion, LFR) as the performance of AutoML remains well above random guess at many or all settings of $\gamma$.
These results experimentally confirm the theoretical impossibility theorem of Section \ref{sec:challenge}, and are of particular concern as they regard models that take overall fair allocation decisions. 
For instance, the DebiasClassifier is able to learn fair allocations on COMPAS; however, the representations still contain information about $S$ and should therefore not be considered safe for distribution to data users interested in employing them in other ML tasks.
We give a comparison of a ReLU-activated DebiasClassifier in the Appendix, Section~\ref{sec:app-relu}, where we observe similarly that information is not consistently removed.
A similar trend is clearly visible for the NVP model across all datasets.

We conclude by offering an explanation for the phenomenon of fair allocation models not learning invariant representations. 
We note that the observation that when $S$ and $Y$ are correlated, a weak classification model will also be relatively fair in terms of allocation.
Thus, FRL methodologies which are not severely tested for representation invariance may still obtain fair allocation decisions via a weak classification stage $Z^i \to \hat{Y}$.
%
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{plots/automl_ACC_pure_gamma_results_relu_False.pdf}
    \caption{AutoML ACC vs. gamma results for all six dataset and eight model combinations.}
    \label{fig:automl-auc}
\end{figure}

